Utilising the CLT Structure in Stochastic Gradient based Sampling : Improved Analysis and Faster Algorithms

We consider stochastic approximations of sampling algorithms, such as Stochastic Gradient Langevin Dynamics (SGLD) and the Random Batch Method (RBM) for Interacting Particle Dynamcs (IPD). We observe that the noise introduced by the stochastic approximation is nearly Gaussian due to the Central Limit Theorem (CLT) while the driving Brownian motion is exactly Gaussian. We harness this structure to absorb the stochastic approximation error inside the diffusion process, and obtain improved convergence guarantees for these algorithms. For SGLD, we prove the first stable convergence rate in KL divergence without requiring uniform warm start, assuming the target density satisfies a Log-Sobolev Inequality. Our result implies superior first-order oracle complexity compared to prior works, under significantly milder assumptions. We also prove the first guarantees for SGLD under even weaker conditions such as H\"{o}lder smoothness and Poincare Inequality, thus bridging the gap between the state-of-the-art guarantees for LMC and SGLD. Our analysis motivates a new algorithm called covariance correction, which corrects for the additional noise introduced by the stochastic approximation by rescaling the strength of the diffusion. Finally, we apply our techniques to analyze RBM, and significantly improve upon the guarantees in prior works (such as removing exponential dependence on horizon), under minimal assumptions.

==> redundancies.tex <==
\subsection{Contributions}

\paragraph{Improved Convergence of SGLD with Log-Sobolev} When $\pistar$ satisfies a log-Sobolev inequality, $\nabla F$ is smooth and every point on the trajectory has finite $4$-th  moment of the order $d^2$, we obtain a first-order oracle complexity of $O\left(\frac{d^{3/2}}{\epsilon^2}\right)$ to ensure that the KL-divergence to the target is $\leq \epsilon^2$. We relax the 4-th moment assumption in the finite sum setting by considering adaptive batch sizes. Our results improve upon the previous state-of-the-art results (\cite{quanquan-sgld}) for SGLD by improving the oracle complexity by a factor of $d^{2.5}$, removing the assumptions of dissipativity and uniform warm start. Moreover, unlike prior works \citep{quanquan-sgld,raginsky2017non}, our  guarantees are stable (i.e., they do not diverge as the number of iterations grows to infinity). Our results show an improvement even over variance reduced SGLD \cite{suzuki-VR-SGLD-2022} which achieves an oracle complexity of $\frac{\sqrt{n}d}{\epsilon^2}$ for finite sum minimization with $n$ terms. This is in firm contrast to optimization where variance reduced methods outperform vanilla stochastic gradient descent (SGD)(\cite{johnson2013accelerating,defazio2014saga,schmidt2017minimizing}). 





\paragraph{First-Order Stationarity and Guarantees under Poincare Inequality for SGLD} In the absence of any isoperimetric assumptions on $\pistar$, we obtain stable $\Otilde(\nicefrac{d^{2.5}}{\epsilon^2})$ oracle complexity guarantee for $\epsilon$-convergence in Fisher Divergence. 


for the average law of SGLD with respect to Fisher Divergence, assuming $F$ is smooth and the SGLD trajectory has $O(d^2)$ fourth moments. Since convergence in Fisher Divergence in sampling is analogous to first order stationarity in nonconvex optimization \citep{sinho-non-log-concave-lmc, sinho-fisher-lb}, we essentially establish the first 

We derive convergence guarantees for the average law of SGLD with respect to Fisher Divergence, assuming smoothness of $F$, and $O(d^2)$ fourth moments of the trajectory. without making any isoperimetric assumptions on $\pistar$
 We derive convergence guarantees for the average law of SGLD iterates with respect to the Fisher Divergence without any isoperimetry assumptions on $\pistar$. In the process, we also obtain the first known stable guarantee for SGLD under Poincare Inequality.
 \anant{commenting out the rest} %This implies convergence under the TV distance if $\pistar$ satisfies a Poincare inequality, giving us the first known stable guarantee for SGLD under the Poincare Inequality. Such bounds have been recently considered for LMC \citep{sinho-non-log-concave-lmc, sinho-fisher-lb}.


 %In fact, by appealing to the interpretation of sampling as optimization over the space of measures, \cite{sinho-non-log-concave-lmc} motivate convergence analysis in Fisher Divergence to be the non-logconcave sampling analog of (first order) stationary-point analysis in nonconvex optimization, and along these lines, establish stationarity guarantees for the law  of averaged LMC. Thus, we extend this line of work by establishing the first known stationarity guarantees of SGLD for smooth non-logconcave sampling. As before, our guarantees are stable and do not require any uniform warm start assumption. Furthermore, we show that our Fisher Divergence guarantees imply stable convergence of averaged SGLD in Total Variation if $\pistar$ satisfies a Poincare inequality. To the best of our knowledge, this is the first known stable guarantee for SGLD under the Poincare Inequality.

% The previous state-of-the-art results for SGLD by \cite{quanquan-sgld} achieved a first order oracle complexity of $\frac{d^4}{\epsilon^2}$ under the stronger assumption of dissipativity and uniform warm start (uniform bound on the Radon-Nikodym derivative of the initial distribution with respect to the target). Moreover, they achieve a stochastic gradient complexity of to ensure total variation distance to the target $\mathsf{TV} \leq \epsilon$, which is weaker compared to $\mathsf{KL} \leq \epsilon^2$. 

\anant{commenting out this}
% For a finite sum $ F(x) = \frac{1}{n}\sum_{i=1}^{n}f_i(x)$, LMC has the first order oracle complexity of $O(\frac{nd}{\epsilon^2})$ \cite{vempalawibisono19} and variance reduced SGLD (\cite{suzuki-VR-SGLD-2022}) has the complexity of $\frac{\sqrt{n}d}{\epsilon^2}$ (best known upper bounds). This is in firm contrast to optimization where variance reduced methods outperform vanilla stochastic gradient descent (SGD)(\cite{johnson2013accelerating,defazio2014saga,schmidt2017minimizing}). 


\begin{center}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    Paper & Assumptions & Metric & Rates & Stability \\
    \hline
       \cite{raginsky2017non}   &              &        &   &         \\
    \hline
       \cite{quanquan-sgld}   &              &          &   &            \\
    \hline
        Our Work  &              &      &   &        \\
    \hline
    \end{tabular}
\end{center}
%\ad{TRIPLE CHECK THIS. We are better than \cite{quanquan-sgld} for sure. AFAIK there hasn't been any major leaps since then without strong assumptions like warm start}
% Furthermore, by use of standard information-transport inequalities, we show that our results imply state-of-the-art convergence guarantees for SGLD with respect to the Total Variation metric as well as Wasserstein distance. 
 % \dn{explain first order oracle}

 % \dn{ I have commented out some content written before, please do add some of that content here. We should not add too many paragraphs in contributions it will just end up confusing the reader. We will add some of the commented discussion into `proof technique' or `proof overview instead of contribution'. We also need a very nice table - in the table, compare to LMC, other bounds, SVRG based bounds}

 %We observe that the noise introduced by the stochastic gradients in SGLD has a CLT structure, i.e., it is a sum of zero-mean i.i.d random variables, and demonstrate that, by appropriately utilizing this CLT structure, one can effectively \emph{absorb the error due to stochastic approximation within the Brownian motion} term of SGLD. Hiding the stochastic gradient noise in the Brownian motion allows us to analyze SGLD via the \emph{interpolation method}, a popular technique developed by \cite{vempalawibisono19} which is used by several subsequent works for analyzing LMC and its variants \citep{wibisono-proximal-ula,sinho-lmc-poincare-lsi, sinho-non-log-concave-lmc}. In particular, we construct a piecewise continuous stochastic process that interpolates the discrete-time trajectory of SGLD. Subsequently, by analyzing the time evolution of the KL divergence along this process, we obtain a discrete-time Evolution Variational Inequality (or EVI) for SGLD, which allows us to prove nonasymptotic convergence guarantees under a variety of settings.   


% \paragraph{Stable Convergence of SGLD in KL under LSI} Under the assumption that $\pistar$ satisfies a Log Sobolev Inequality (LSI), we recast the obtained EVI into a descent lemma for the KL divergence. Subsequently, we derive convergence guarantees for SGLD with respect to the KL divergence between the law of the last iterate and the target distribution. Unlike prior works \citep{quanquan-sgld,raginsky2017non}, our  guarantees are stable (i.e., they do not diverge as the number of iterations grows to inifinity) and also do not require any uniform warm start assumption. Furthermore, by use of standard information-transport inequalities, we show that our results imply state-of-the-art convergence guarantees for SGLD with respect to the Total Variation metric as well as Wasserstein distance. \ad{TRIPLE CHECK THIS. We are better than \cite{quanquan-sgld} for sure. AFAIK there hasn't been any major leaps since then without strong assumptions like warm start}  

\paragraph{First-Order Stationarity and Guarantees under Poincare Inequality for SGLD}
 We derive convergence guarantees for the average law of SGLD iterates with respect to the Fisher Divergence without any isoperimetry assumptions on $\pistar$. In the process, we also obtain the first known stable guarantee for SGLD under Poincare Inequality.
 \anant{commenting out the rest} %This implies convergence under the TV distance if $\pistar$ satisfies a Poincare inequality, giving us the first known stable guarantee for SGLD under the Poincare Inequality. Such bounds have been recently considered for LMC \citep{sinho-non-log-concave-lmc, sinho-fisher-lb}.


 %In fact, by appealing to the interpretation of sampling as optimization over the space of measures, \cite{sinho-non-log-concave-lmc} motivate convergence analysis in Fisher Divergence to be the non-logconcave sampling analog of (first order) stationary-point analysis in nonconvex optimization, and along these lines, establish stationarity guarantees for the law  of averaged LMC. Thus, we extend this line of work by establishing the first known stationarity guarantees of SGLD for smooth non-logconcave sampling. As before, our guarantees are stable and do not require any uniform warm start assumption. Furthermore, we show that our Fisher Divergence guarantees imply stable convergence of averaged SGLD in Total Variation if $\pistar$ satisfies a Poincare inequality. To the best of our knowledge, this is the first known stable guarantee for SGLD under the Poincare Inequality. 

\paragraph{ SGLD Analysis via Entropic CLT } 
We derive a novel entropic central limit theorem to quantify the approximate Gaussianity of the stochastic gradient noise in SGLD. This allows us to obtain KL upper bounds between the trajectories of LMC and SGLD, by only assuming that the iterates of LMC has finite 6-th moments of the order $d^3$ (and without any functional inequality assumptions). % This allows us to conclude that the convergence of LMC is (nearly) a sufficient condition for SGLD to converge under the same setting, and nearly at the same rate.

We prove the first last iterate TV-convergence of SGLD under the assumption that $\pistar$ satisfies either a Lata\l{}a-Oleskiewicz (LO) Inequality a Modified Log Sobolev Inequality (MLSI). LMC was analyzed recently under these conditions \citep{murat-mlsi-paper, sinho-lmc-poincare-lsi}.  

%%%Furthermore, our entropic CLT may be of independent interest for analyzing stochastic approximations of more sophisticated sampling and optimization algorithms. %To the best of our knowledge, our results are the first to establish the last iterate convergence of SGLD under this setting.
%trajectories of \emph{SGLD is nearly statistically indistinguishable from LMC} by deriving upper bounds for the KL divergence between the trajectories of SGLD and LMC. A key component of our proof is a novel entropic central limit theorem that quantifies the approximate Gaussianity of the stochastic gradient noise in SGLD. Our statistical indistinguishability result does not rely on any functional inequality assumption on $\pistar$, nor does it require any uniform warm start. This allows us to conclude that the convergence of LMC is (nearly) a sufficient condition for SGLD to converge under the same setting, and nearly at the same rate (modulo some residual error terms due to stochastic approximation). To quantitatively establish this, we use our statistical indistinguishability guarantees to prove the convergence of the law of the last iterate of SGLD with respect to the Total Variation metric, under the assumption that $\pistar$ satisfies either a Lata\l{}a-Oleskiewicz (LO) Inequality \citep{latala-oleskiewicz-paper} or a Modified Log Sobolev Inequality (MLSI) \citep{murat-mlsi-paper}. These inequalities interpolate between the Poincare and Log Sobolev inequalities, and were considered in recent works \citep{murat-mlsi-paper, sinho-lmc-poincare-lsi} for analyzing LMC under weak functional inequality assumptions. To the best of our knowledge, our results are the first to establish the last iterate convergence of SGLD under this setting. Furthermore, our entropic CLT may be of independent interest for analyzing stochastic approximations of more sophisticated sampling and optimization algorithms. 


\paragraph{Covariance Correction for SGLD} Based on the entropic CLT discussed above, we design a novel algorithmc called covariance corrected SGLD (CC-SGLD).   CC-SGLD enjoys an improved first order oracle complexity of 
$O(\frac{d^{4/3}}{\epsilon^2})$ under additional conditions. \anant{commenting this out}%As discussed above, optimization style variance reduction ported to SGLD has much worse convergence bounds than vanilla SGLD. This provides some evidence that variance reduction in sampling algorithms are inherently differently from those in optimization algorithms. 

%The correction is made in a manner such that Covariance Corrected SGLD (or CC-SGLD) admits the same random function representation as that of LMC. To this end, we apply our entropic CLT analysis to CC-SGLD and show that the KL divergence between the trajectories of CC-SGLD and LMC is less than that between SGLD and LMC. As before, our statistical indistinguishability guarantee neither relies on any functional inequality assumptions on $\pistar$, nor does it require any uniform warm start. Subsequently, we show that this improved statistical indistinguishability (compared to SGLD without covariance correction) leads to faster convergence of CC-SGLD in a variety of settings. 

\paragraph{Random Batch Method for IPD} We consider the  Random batch method (RBM) and
Covariance Corrected Random Batch Method (CC-RBM) for IPD. We show that after for a simulation with $K$ steps, step-size $\eta$, $n$ particles, and batch size $B$, RBM incurs a KL divergence error of $O(\frac{n\alpha^2 K}{B^2})$ to IPD, and CC-RBM incurs $O(\frac{n\alpha^2 K}{B^3})$. Our work improves upon the stringent assumptions in prior works on the confining and interaction potentials (anti-derivatives of $\vg_k^{ij}$ and $\vK_k^{ij}$ in \ref{eqn:IPD}). \cite{jin2020random} assumes that the confining potential is strongly convex and the interaction potentials are lipschitz, with the lipschitz constant being small enough compared to the strong-convexity parameter. While \cite{jin2021convergence} relaxes the strong-convexity assumption, the bounds suffer from an exponential dependence on $\eta K$.



\section{Analysis of SGLD via Entropic CLT}
In this section, we prove a \emph{statistical indistinguishability} guarantee between SGLD and LMC without any smoothness or functional inequality assumptions on the target. We use $(\vx_k)_{k \in (K)}$ to denote the iterates of LMC, which satisfy the following update equation,
\begin{align*}
    \vx_{k+1} = \vx_k - \eta \nabla F(\vx_k) + \sqrt{2 \eta} \epsilon_k, \ \epsilon_k \sim \cN(0, \vI)
\end{align*}
The key result of this section establishes that, under minimal assumptions, the trajectory $(\hvx_k)_{k \in (K)}$ of SGLD is statistically indistinguishable with respect to the KL divergence, from that of $(\vx_k)_{k \in (K)}$ of LMC. Our proof relies on two key intuitions: 1. Assuming same step-sizes and initialization, SGLD and LMC admit the same random function representation, 2. The noise introduced by the stochastic approximation in SGLD can be effectively \emph{hidden inside the Gaussian noise} introduced by the Brownian motion. To this end, an important technical tool of our analysis is the following Wasserstein CLT for Gaussian convolutions of bounded random vectors, which may be of independent interest for analyzing stochastic approximations of sampling and optimization algorithms. We present a proof of this lemma in Appendix \ref{proof:lem-wass-clt-new}
\begin{comment}
\begin{lemma}[$\wass{2}$ CLT for Gaussian Convolutions of Bounded RVs]
\label{lem:wass-clt-new}
Let $\vY_1, \dots, \vY_B$ be i.i.d random vectors in $\bR^d$ satisfying $\bE\left[ \vY_i \right] = 0$, $\bE \left[\vY_i \vY^T_i \right] = \Sigma_{\vY}$ and $\norm{\vY_i} \leq \beta$ almost surely, and let $\vY = \frac{1}{\sqrt{B}} \sum_{i=1}^{B} \vY_i$. Furthermore, let $\vX$ and $\vZ$ be sampled iid from $\cN(0, \vI)$, independent of $\vY_1, \dots, \vY_B$. Then, the following holds for $\beta^2 \leq \nicefrac{1}{5}$ and $\norm{\Sigma_{\vY}}_2 \leq \nicefrac{1}{5d}$
\begin{align*}
    \wass{2}^2(\sqrt{\vI - \Sigma_{\vY}}\vX + \vY,  \vZ) = \frac{25 \beta^6 d (1 + \log(B))}{B}
\end{align*}
\end{lemma}
Lemma \ref{lem:wass-clt-new} allows us to quantitatively hide the stochastic gradient noise of SGLD within the Brownian motion. Equipped with this tool, we prove the following statistical indistinguishability guarantee, whose proof is presented in Appendix \ref{proof:thm-sgld-stat-indistinguishable}
\begin{theorem}[Statistical Indistinguishability of SGLD and LMC]
\label{thm:sgld-stat-indistinguishable}
Let the \ref{eqn:defn-grad-growth} and \ref{eqn:defn-moment-growth} conditions be satisfied with $p = 6\zeta$. Then, the iterates of SGLD satisfy the following guarantee 
\begin{align*}
    \KL{\hvx_{1:K}}{\vx_{1:K}} &\leq \frac{2 \eta^2 K}{B^2} \left(M^{4} C_{4\zeta} d^{2\zeta} + G^{4\zeta}\right) + \frac{3000 \eta^3 K}{B^4}\left(M^{6} C_{6 \zeta} d^{3\zeta + 3} + G^{6} d^3 \right)\left(1 + \log B \right)^2
\end{align*}
\end{theorem}
\end{comment}

Theorem \ref{thm:sgld-stat-indistinguishable} establishes that, under appropriate choices of $B, \eta$ and $K$, no statistical test can distinguish the paths generated by SGLD from that of LMC. As a consequence, it implies that \emph{the convergence of LMC to the target distribution $\pistar$ is nearly sufficient to ensure the convergence of SGLD to $\pistar$}. To illustrate this quantitatively, we use Theorem \ref{thm:sgld-stat-indistinguishable} to establish the first known convergence guarantee of SGLD under the mild assumptions of \ref{eqn:defn-holder-smoothness} and \ref{eqn:defn-latala-oleskiewicz} for any $s \in (\nicefrac{1}{2}, 1]$ and $\alpha \in [1,2]$. \ad{We should highlight that this is only one possible example. In general, Theorem \ref{thm:sgld-stat-indistinguishable} gives a general recipe for proving SGLD convergence bounds, that would automatically adapt to future advancements in the analysis of LMC}


\section{Covariance Corrected SGLD}
% The key insight from our analysis of SGLD is the fact that the noise added by the stochastic gradients, due to its CLT structure, exhibits approximate Gaussianity, and thus, can be absorbed into the Brownian motion term, whose increments are exactly Gaussian. This insight naturally suggests that the quality of the stochastic approximation could be improved if the excess noise introduced by the stochastic gradients could be compensated for by appropriately adjusting the strength of the diffusion term. To this end, we develop \emph{Covariance Correction} for SGLD, which involves estimating the covariance of the stochastic gradient noise (using a fresh batch of samples) and appropriately adjusting the diffusion term of the update. The resulting algorithm, called Covariance Corrected SGLD (or CC-SGLD) is described as follows. 
% \anant{AR: add  algorithm environment}
% \begin{enumerate}
%     \item Sample a batch of stochastic gradients $\nabla f(\hvx_k, \xi_{k, 1}), \dots, \nabla f(\hvx_k, \xi_{k, B})$ and compute $\vg_k = \nicefrac{1}{B} \sum_{j=1}^{B} \nabla f(\hvx_k, \xi_{k, j})$ 
%     \item If $M \norm{\hvx_k}^{\zeta} + G > \nicefrac{B}{5 \eta d}$, then sample $\hvw_k \sim \cN(0, \vI)$ and skip to step 4
%     \item Otherwise, sample another batch  $\nabla f(\hvx_k, \xi^{(1)}_{k, 1}), \nabla f(\hvx_k, \xi^{(2)}_{k, 1}), \dots, \nabla f(\hvx_k, \xi^{(1)}_{k, B}),  \nabla f(\hvx_k, \xi^{(2)}_{k, B})$ and compute $\hSigma_k$ as
%     \begin{align*}
%         \hSigma_k &= \nicefrac{1}{2B^2} \sum_{j=1}^{B} \left(\nabla f(\vx_k, \xi^{(1)}_{k, j}) - \nabla f(\vx_k, \xi^{(2)}_{k, j})\right) \left(\nabla f\nabla f(\vx_k, \xi^{(1)}_{k, j}) - \nabla f(\vx_k, \xi^{(2)}_{k, j})\right)^{T}
%     \end{align*}
%     Set $\hvw_k = \sqrt{\vI - \nicefrac{\eta}{2}\hSigma_k} \heps_k, \ \heps_k \sim \cN(0, \vI)$
%     \item Compute the update as follows
%     \begin{align*}
%         \hvx_{k+1} \leftarrow \hvx_k - \eta \vg_k + \sqrt{2 \eta} \hvw_k
%     \end{align*}
% \end{enumerate}
In the following theorem, whose proof we present in Appendix \ref{proof:thm-cc-sgld-stat-indistinguishable}, we show that Covariance Corrected SGLD is a better stochastic approximation of LMC than ordinary SGLD. 
By comparing with Theorem \ref{thm:sgld-stat-indistinguishable}, we observe that incorporating covariance correction in SGLD leads to an improved statistical indistinguishability guarantee compared to ordinary SGLD, thereby leading to improved convergence. We establish this under the mild assumptions of \ref{eqn:defn-holder-smoothness} and \ref{eqn:defn-latala-oleskiewicz} for any $s \in [\nicefrac{1}{2}, 1]$ and $\alpha \in [1, 2]$. The proof is deferred to Appendix \ref{cor:cc-sgld-unstable-lo}. 
\ad{Need to be more careful about choice of the batch size here otherwise improvement over CC-SGLD is not always apparent for $s < 1$}

Since $\zeta \geq \nicefrac{1}{2}$, one can observe that CC-SGLD has a better oracle complexity compared to that ordinary SGLD in the same setting as implied by Corollary \ref{cor:sgld-unstable-lo}. For ease of exposition, we explicitly illustrate this for the specific cases of of \ref{eqn:defn-log-sobolev} and \ref{eqn:defn-poincare} under the \ref{eqn:defn-smoothness} assumption.

\paragraph{Rates Under LSI} For $\alpha = 2$ and $s = 1$, which corresponds to the \ref{eqn:defn-smoothness} and \ref{eqn:defn-log-sobolev} case, Corollary \ref{cor:cc-sgld-unstable-lo} implies an oracle complexity of $\Thetatilde(\frac{d^{\nicefrac{2}{3}\left(\zeta + 1\right)}}{\epsilon^2})$ for last-iterate $\epsilon$-convergence in $\TV$. In the worst case, the oracle complexity becomes $\Thetatilde(\frac{d^{\nicefrac{4}{3}}}{\epsilon^2})$ for $\zeta = 1$. We note that this improves upon the guarantees of Corollary \ref{cor:sgld-unstable-lo} as well as Theorems \ref{thm:sgld-lsi-stable} and \ref{thm:absgld-lsi-stable} under the same setting. However, unlike Theorems \ref{thm:sgld-lsi-stable} and \ref{thm:absgld-lsi-stable}, the guarantee established by \ref{cor:cc-sgld-unstable-lo} is an unstable convergence guarantee

\paragraph{Rates Under PI} For $\alpha = 1$ and $s = 1$, which corresponds to the \ref{eqn:defn-smoothness} and \ref{eqn:defn-poincare} case, Corollary \ref{cor:cc-sgld-unstable-lo} implies an oracle complexity of $\Thetatilde(\frac{d^{\nicefrac{2}{3}\left(\epsilon + 4\right)}}{\epsilon^2})$ rate for $\epsilon$-convergence in TV. The worst case complexity for $\zeta = 1$ is $\Thetatilde(\frac{d^{\nicefrac{10}{3}}}{\epsilon^2})$. We note that this improves upon the guarantee implied by Corollary \ref{cor:sgld-unstable-lo} in the same setting. When compared to the $\Otilde\left(\frac{d^{\zeta + \nicefrac{3}{2}}}{\epsilon^4}\right)$ guarantee of \emph{averaged LMC} implied by \ref{thm:sgld-fd-and-pi}, we note that Corollary \ref{cor:cc-sgld-unstable-lo} exhibits a better dependence on $\epsilon$ at the cost of a worse dimension dependence.  
\begin{comment}
\paragraph{Rates Under LSI without Smoothness \ad{Rewrite this. LSI implies smoothness}} Since the LO inequality with $\alpha = 2$ is equivalent to LSI, we conclude that Corollary \ref{cor:sgld-unstable-lo} implies an oracle complexity of $\Tilde{\Theta}\left(\frac{d^{ s + \nicefrac{1}{2}}}{\epsilon^{\nicefrac{2}{s}}}\right)$ to ensure $\epsilon$-convergence in TV for the last iterate. To the best of our knowledge, this is the first known result for SGLD under LSI without any smoothness assumption. To compare with Theorem \ref{thm:sgld-lsi-stable}, we observe that the setting $s = 1$ has an oracle complexity $\Tilde{\Theta}(\nicefrac{d^{\nicefrac{3}{2}}}{\epsilon^2})$ of which matches the guarantee implied by \ref{thm:sgld-lsi-stable} via an application of Pinsker's Inequality. However, we emphasize that Theorem \ref{thm:sgld-lsi-stable} is a stronger result as it implies convergence in a stronger metric (i.e. KL divergence), and, unlike Corollary \ref{cor:sgld-unstable-lo}, is a stable convergence guarantee. 

\paragraph{Last-Iterate Convergence Under PI} Since the LO inequality with $\alpha = 1$ is equivalent to the Poincare Inequality, we conclude that Corollary \ref{cor:sgld-unstable-lo} implies an oracle complexity of $\Tilde{\Theta}\left(\frac{d^{s + 2 + \nicefrac{1}{2s}}}{\epsilon^{\nicefrac{2}{s}}}\right)$ to ensure $\epsilon$-convergence in TV for the last iterate. To the best of our knowledge, this is the first known result for the last-iterate SGLD under PI, as well as the first known result for SGLD under PI without any smoothness assumption. We note that the setting $s = 1$ has an oracle complexity $\Tilde{\Theta}(\nicefrac{d^{\nicefrac{7}{2}}}{\epsilon^2})$ to ensure $\epsilon$-convergence for the last iterate. On the contrary, Theorem \ref{thm:sgld-fd-and-pi} requires $\Tilde{\Theta}(\nicefrac{d^{\nicefrac{5}{2}}}{\epsilon^4})$ oracle calls to ensure the same for the average iterate. Thus, the guarantee implied by Corollary \ref{cor:sgld-unstable-lo} in this setting is better than that of \ref{thm:sgld-fd-and-pi} in terms of $\epsilon$ dependence at the cost of a worse $d$ dependence. However, we emphasize that, unlike Corollary \ref{cor:sgld-unstable-lo}, Theorem \ref{thm:sgld-fd-and-pi} presents a stable convergence guarantee. 
\end{comment}
\section{Analysis of Random Batch Method for Interacting Particle Dynamics}
To demonstrate that our CLT analysis techniques are not restricted to SGLD, we now consider the Random Batch Method for interacting particle systems, which involves a stochastic approximation of the inter-particle interactions. In particular, we observe that the update equations of RBM can be expressed as follows,
\begin{align*}
    \hvx^{i}_{k+1} &= \hvx^{i}_k - \eta \vg_k(\hvx^{i}_k) + \frac{\eta}{n}\sum_{j=1}^{n} \vK^{ij}_{k}(\hvx^{k}_i, \hvx^{k}_j) + \sigma \sqrt{\eta} \hvz^{i}_k \\
    \hvz^{i}_k &= \nicefrac{\sqrt{\eta}}{\sigma}\vN^i_k + \heps^k_i, \ \ \heps^k_i \sim \cN(0, \vI)
\end{align*}
where $\vN^i_k$ is the noise due to stochastic approximation of the inter-particle interactions
\begin{align*}
    \vN^i_k  = \frac{1}{B} \sum_{j=1}^{B}\left[ \vK^{i I^{ij}_k}_{k}(\hvx^i_k, \hvx^{I^{ij}_k}_k) - \frac{1}{n} \sum_{l=1}^{n} \vK^{il}_{k}(\hvx^{k}_i, \hvx^{k}_l)  \right]
\end{align*}
Since $I^{ij}_k \ \iidsim \ \mathsf{Uniform}([n])$, we observe that $\vN^i_k$ admits a CLT structure, and hence, is approximately Gaussian. Furthermore, we note that IPD and RBM admit the same random function representation. Thus, our entropic CLT analysis of SGLD can be directly applied to establish the following statistical indistinguishability guarantee between IPD and RBM, 
In a similar fashion, we note that the Covariance Corrected Random Batch Method admits the same random function representation as IPD, when expressed as follows,
\begin{align*}
    \hvx^{i}_{k+1} &= \hvx^{i}_k - \eta \vg_k(\hvx^{i}_k) + \frac{\eta}{n}\sum_{j=1}^{n} \vK^{ij}_{k}(\hvx^{k}_i, \hvx^{k}_j) + \sigma \sqrt{\eta} \hvz^{i}_k \\
    \hvz^{i}_k &= \nicefrac{\sqrt{\eta}}{\sigma}\vN^i_k + \sqrt{\vI - \nicefrac{\eta}{\sigma^2} \hSigma^i_k}\heps^k_i, \ \ \heps^k_i \sim \cN(0, \vI)
\end{align*}
where $\vN^i_k$ is as defined above. Consequently, using the same techniques as our analysis of CC-SGLD in Theorem \ref{thm:cc-sgld-stat-indistinguishable}, we establish that CC-RBM is an improved stochastic approximation of IPD. We prove this result in Appendix \ref{proof:thm-cc-rbm-stat-indistinguishability}.



% The previous state-of-the-art results for SGLD by \cite{quanquan-sgld} achieved a first order oracle complexity of $\frac{d^4}{\epsilon^2}$ under the stronger assumption of dissipativity and uniform warm start (uniform bound on the Radon-Nikodym derivative of the initial distribution with respect to the target). Moreover, they achieve a stochastic gradient complexity of to ensure total variation distance to the target $\mathsf{TV} \leq \epsilon$, which is weaker compared to $\mathsf{KL} \leq \epsilon^2$. 

%\anant{commenting out this}
% For a finite sum $ F(x) = \frac{1}{n}\sum_{i=1}^{n}f_i(x)$, LMC has the first order oracle complexity of $O(\frac{nd}{\epsilon^2})$ \cite{vempalawibisono19} and variance reduced SGLD (\cite{suzuki-VR-SGLD-2022}) has the complexity of $\frac{\sqrt{n}d}{\epsilon^2}$ (best known upper bounds). This is in firm contrast to optimization where variance reduced methods outperform vanilla stochastic gradient descent (SGD)(\cite{johnson2013accelerating,defazio2014saga,schmidt2017minimizing}). 


% \begin{center}
%     \begin{tabular}{|c|c|c|c|c|}
%     \hline
%     Paper & Assumptions & Metric & Rates & Stability \\
%     \hline
%        \cite{raginsky2017non}   &              &        &   &         \\
%     \hline
%        \cite{quanquan-sgld}   &              &          &   &            \\
%     \hline
%         Our Work  &              &      &   &        \\
%     \hline
%     \end{tabular}
% \end{center}
%\ad{TRIPLE CHECK THIS. We are better than \cite{quanquan-sgld} for sure. AFAIK there hasn't been any major leaps since then without strong assumptions like warm start}
% Furthermore, by use of standard information-transport inequalities, we show that our results imply state-of-the-art convergence guarantees for SGLD with respect to the Total Variation metric as well as Wasserstein distance. 
 % \dn{explain first order oracle}

 % \dn{ I have commented out some content written before, please do add some of that content here. We should not add too many paragraphs in contributions it will just end up confusing the reader. We will add some of the commented discussion into `proof technique' or `proof overview instead of contribution'. We also need a very nice table - in the table, compare to LMC, other bounds, SVRG based bounds}

 %We observe that the noise introduced by the stochastic gradients in SGLD has a CLT structure, i.e., it is a sum of zero-mean i.i.d random variables, and demonstrate that, by appropriately utilizing this CLT structure, one can effectively \emph{absorb the error due to stochastic approximation within the Brownian motion} term of SGLD. Hiding the stochastic gradient noise in the Brownian motion allows us to analyze SGLD via the \emph{interpolation method}, a popular technique developed by \cite{vempalawibisono19} which is used by several subsequent works for analyzing LMC and its variants \citep{wibisono-proximal-ula,sinho-lmc-poincare-lsi, sinho-non-log-concave-lmc}. In particular, we construct a piecewise continuous stochastic process that interpolates the discrete-time trajectory of SGLD. Subsequently, by analyzing the time evolution of the KL divergence along this process, we obtain a discrete-time Evolution Variational Inequality (or EVI) for SGLD, which allows us to prove nonasymptotic convergence guarantees under a variety of settings.   


% \paragraph{Stable Convergence of SGLD in KL under LSI} Under the assumption that $\pistar$ satisfies a Log Sobolev Inequality (LSI), we recast the obtained EVI into a descent lemma for the KL divergence. Subsequently, we derive convergence guarantees for SGLD with respect to the KL divergence between the law of the last iterate and the target distribution. Unlike prior works \citep{quanquan-sgld,raginsky2017non}, our  guarantees are stable (i.e., they do not diverge as the number of iterations grows to inifinity) and also do not require any uniform warm start assumption. Furthermore, by use of standard information-transport inequalities, we show that our results imply state-of-the-art convergence guarantees for SGLD with respect to the Total Variation metric as well as Wasserstein distance. \ad{TRIPLE CHECK THIS. We are better than \cite{quanquan-sgld} for sure. AFAIK there hasn't been any major leaps since then without strong assumptions like warm start}  

  

%%%Furthermore, our entropic CLT may be of independent interest for analyzing stochastic approximations of more sophisticated sampling and optimization algorithms. %To the best of our knowledge, our results are the first to establish the last iterate convergence of SGLD under this setting.
%trajectories of \emph{SGLD is nearly statistically indistinguishable from LMC} by deriving upper bounds for the KL divergence between the trajectories of SGLD and LMC. A key component of our proof is a novel entropic central limit theorem that quantifies the approximate Gaussianity of the stochastic gradient noise in SGLD. Our statistical indistinguishability result does not rely on any functional inequality assumption on $\pistar$, nor does it require any uniform warm start. This allows us to conclude that the convergence of LMC is (nearly) a sufficient condition for SGLD to converge under the same setting, and nearly at the same rate (modulo some residual error terms due to stochastic approximation). To quantitatively establish this, we use our statistical indistinguishability guarantees to prove the convergence of the law of the last iterate of SGLD with respect to the Total Variation metric, under the assumption that $\pistar$ satisfies either a Lata\l{}a-Oleskiewicz (LO) Inequality \citep{latala-oleskiewicz-paper} or a Modified Log Sobolev Inequality (MLSI) \citep{murat-mlsi-paper}. These inequalities interpolate between the Poincare and Log Sobolev inequalities, and were considered in recent works \citep{murat-mlsi-paper, sinho-lmc-poincare-lsi} for analyzing LMC under weak functional inequality assumptions. To the best of our knowledge, our results are the first to establish the last iterate convergence of SGLD under this setting. Furthermore, our entropic CLT may be of independent interest for analyzing stochastic approximations of more sophisticated sampling and optimization algorithms. 
